Thermal emission from the amorphous dust: An alternative possibility of the origin of the anomalous microwave emission

Complete studies of the radiative processes of thermal emission from the amorphous dust from microwave through far infrared wavebands are presented by taking into account, self-consistently for the first time, the standard two-level systems (TLS) model of amorphous materials. The observed spectral energy distributions (SEDs) for the Perseus molecular cloud (MC) and W43 from microwave through far infrared are fitted with the SEDs calculated with the TLS model of amorphous silicate. We have found that the model SEDs well reproduce the observed properties of the anomalous microwave emission (AME). The present result suggests an alternative interpretation for the AME being carried by the resonance emission of the TLS of amorphous materials without introducing new species. Simultaneous fitting of the intensity and polarization SEDs for the Perseus MC and W43 are also performed. The amorphous model reproduces the overall observed feature of the intensity and polarization SEDs of the Perseus MC and W43. However, the model's predicted polarization fraction of the AME is slightly higher than the QUIJOTE upper limits in several frequency bands. A possible improvement of our model to resolve this problem is proposed. Our model predicts that interstellar dust is amorphous materials having very different physical characteristics compared with terrestrial amorphous materials.

==> AME.tex <==
\section{Anomalous microwave emission}
\label{sec:AME}

The origin of AME is still under debate.
The spatial correlation between AME and Galactic interstellar dust strongly indicates that AME originates from a kind of dust \citep{Davis+2006}.
The most popular model of the origin of AME is electric dipole emission radiated by charged rotating dust with a frequency of several tens of GHz, as proposed by \citet{Draine+1998};
this is referred to as the spinning dust model.
A carrier of the spinning dust is supposed to be very small grains producing rotation at ultra high frequencies. 
The fact of the lack of AME in cold dense cores supports the spinning dust origin of AME since the lack of the small grains is expected in dense clouds \citep{Tibbs+2016}.
Polycyclic aromatic hydrocarbon (PAH) has been proposed as one of the plausible candidates for spinning dust \citep{Draine+1998}.
However, no observational correlation between amount of PAH and the intensity of AME, as reported by \citet{Hensley+2016}, contradicts the PAH possibility.
A new species of very small dust grains named nanosilicates has been introduced as another possible carrier of the spinning dust (Hoang et al. \yearcite{Hoang+2016}; \cite{Hensley+2017}).
The problem with this possibility is that up to now, apart from AME, no signature to confirm the existence of the nanosilicate has been observed.
The nanosilicate is only observable as AME.
Therefore, it is hard to check whether the carrier of the spinning dust is such a new family of dust grains or not. 
%
%
%
Magnetic dust emission has been proposed as another candidate for the AME mechanism \citep{Draine+1999}.
The spins of electrons inside a magnetic dust grain align spontaneously to settle down to the minimum energy state.
Alignment is disturbed by thermal fluctuation.
Owing to the magnetic relaxation, the disturbed state tries to return to the original minimum energy state.
In course of this transition, microwave radiation is emitted.
This emission could be the origin of AME if the interstellar dust is magnetic \citep{Draine+2013}.
The magnetic dust emission model predicts a positive correlation between the temperature and intensity of AME.
However, \citet{Hensley+2016} found a negative correlation between the AME temperature and intensity that contradicts the predictions of the magnetic dust emission model.
The reported negative correlation is naturally explained by the amorphous model since the intensity of the resonance emission decreases as the dust temperature increases \citep{Meny+2007}.



Crucial clue to distinguishing the emission mechanisms of AME is offered by polarization observations.
\citet{Draine+2016} showed that the quantum effect suppresses the thermalization of the grain rotational kinetic energy of the spinning dust.
As a result, the alignment of grains is suppressed and the spinning dust model predicts a very low degree of polarization.
In the magnetic dust emission model, the high degree of AME polarization  is expected since the main carrier of magnetic dust emission is large grains which are aligned by the interstellar magnetic field.
On the other hand, no study of the polarization emission based on the physical model of the TLS has yet been done.
Although the progress of AME polarization observations have been made by several projects (e.g. WMAP and QUIJOTE), there has as yet been no definite report of the detection of AME polarization (\cite{QUIJOTE1_2015}, \yearcite{QUIJOTE2_2017}).
The detection of polarization from AME has been reported for W43, but whether the reported polarization is a residual of the synchrotron emission of Galactic interstellar matters around W43 is still being debated.
Current observational upper limits somehow rule out the magnetic dust hypothesis, which typically predicts a higher polarization fraction.

